Influencers and the Giant Component: the Fundamental Hardness in Privacy Protection for Socially Contagious Attributes

The presence of correlation is known to make privacy protection more difficult. We investigate the privacy of socially contagious attributes on a network of individuals, where each individual possessing that attribute may influence a number of others into adopting it. We show that for contagions following the Independent Cascade model there exists a giant connected component of infected nodes, containing a constant fraction of all the nodes who all receive the contagion from the same set of sources. We further show that it is extremely hard to hide the existence of this giant connected component if we want to obtain an estimate of the activated users at an acceptable level. Moreover, an adversary possessing this knowledge can predict the real status ("active" or "inactive") with decent probability for many of the individuals regardless of the privacy (perturbation) mechanism used. As a case study, we show that the Wasserstein mechanism, a state-of-the-art privacy mechanism designed specifically for correlated data, introduces a noise with magnitude of order $\Omega(n)$ in the count estimation in our setting. We provide theoretical guarantees for two classes of random networks: Erdos Renyi graphs and Chung-Lu power-law graphs under the Independent Cascade model. Experiments demonstrate that a giant connected component of infected nodes can and does appear in real-world networks and that a simple inference attack can reveal the status of a good fraction of nodes.

==> 04_method.tex <==
% \subsection{Additional Cascade}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figs/secondary.pdf}
%     \caption{Graph partitions before and after the secondary cascade. $v$ is different in $C_1$ and $C_2$.}
%     \label{fig:secondary_cascade}
% \end{figure}
% Let $G^+$ be the subgraph of $G(n,c/n)$ containing all \emph{activated} nodes and all edges connecting them. Let $G^-$ be a similar subgraph for unactivated nodes. We denote the number of nodes in in $G^+$ and $G^-$ by $n^+$ and $n^-$ respectively ($n = n^+ + n^-$). Note that both of these subgraphs are \er~graphs as well. Our proposed randomized algorithm, $\M$, works as follows:

% We select a set of new seeds, $S'$ ($|S'| = k$), uniformly at random from $G^-$ and simulate a new cascade originating from these new nodes over $G^-$. Nodes in $G^+$ report their original $x_i$ values (note that they are all $1$'s), while nodes in $G^-$ report their \emph{new} $x_i$ value resulting from the $k$ additional seed nodes.
% \begin{theorem}\label{theo:puff}
% Suppose that $pq > 1$ and $k = k(n)$ is a function of $n$ that is increasing and $\lim_{n \rightarrow \infty} k(n) = \infty$. The latter is denoted by $k = \omega(1)$. Then,
% $\M$ is $\varepsilon$-Pufferfish. \aria{Details to come}
% \end{theorem}
% \def\cmax{\C_{\text{max}}}
% First, recall that the unactivated subgraph, $G^-$, is also an \er~graph. According to the triggering model for IC, the largest connected component resulting from an IC spread with parameter $q$ is of size $\Theta(n)$ w.h.p. Also, note that the number of randomly selected new seeds, $k$ is $\omega(1)$. In other words: $\lim_{n \rightarrow \infty} k/c = \infty$ for any fixed constant $c > 0$. Suppose that $\cmax$ is the size of the largest connected component of $G^-$, which we will denote by $\cmax$ from now on for notational brevity. For the probability that at least one node $u$ in $\cmax$ is selected as a seed, resulting in activation of the whole connected component, is:
% \begin{align}\label{eq:whp_giant_is_activated}
%     \Pr[S' \cap \cmax \neq \varnothing ] &= 1 - \Pr[S' \cap \cmax = \varnothing] \nonumber\\
%     &= 1 - \prod_{i = 0}^{k - 1}\frac{n^- - \cmax - i}{n^- - i} \nonumber \\
%     &\geq 1 - \left(1 - \frac{\cmax}{n^-}\right)^{k}.
% \end{align}
% Recall that $k = k(n)$ is a function which increases as $n$ grows, with the limit going to infinity. As a result, we can write:
% \begin{equation}
%     \lim_{n \rightarrow \infty} Pr[S' \cap \cmax \neq \varnothing ] \rightarrow 1.
% \end{equation}
% We have now established that if the number of new seeds is an increasing, unbounded function w.r.t $n$, we activate the giant component w.h.p. Now, consider two cascades $\C_1$ and $\C_2$ that differ in the activation status of only one node, $v$. Recall that activation is represented in our problem by $\x_v$, meaning that we can assume that, without loss of generaility, $\x_v(C_1) = 1, \x_v(C_2) = 0$. Suppose that $\M$ produced a secondary cascade, $C$ for $C_1$, i.e. $\M(C_1) = C$. We now prove that when $n$ is sufficiently large, $qp > 1$ and $k = \omega(1)$, with constant probability $\M(C_2)$ also yields $C$. Take out node $v$. Regardless of \emph{how} the secondary cascade spreads throughout $G^-$, we can further divide three subgraph into two smaller ones: the subgraph that includes activated nodes, $H^+$, the subgraph that includes unactivated nodes, $H^-$ and the singular node $v$. Recall that $\x_v(C_1) = 1$ and $\x_v(C_2) = 0$. Note that each instantiation of the cascade happens in $G^+$ with similar probability for both $C_1$ and $C_2$. We only have to calculate the probability that the secondary activation status of $v$, $\x'_v(C_2)$, is equal to $1$ as a result of applying $\M$. In below, we denote $\x'_v(C_2)$ simply by $\x'_v$ for notational brevity.
% \begin{align}\label{eq:same}
%     \Pr[\x'_v = 1, v \not\in S'] &= \Pr[v \not\leftrightarrow u \in H^-]\left(1 - \Pr[v \not\leftrightarrow u \in H^+]\right) \nonumber \\
%     &= \left(1 - \frac{cq}{n}\right)^{|H^-|}\left(1 - \left(1 - \frac{cq}{n}\right)^{|H^+|}\right) \nonumber \\
%     &\geq e^{-cq}\left(1 - e^{-cqy}\right),
% \end{align}
% where $y \in (0, 1)$ is the constant from \eqref{eq:er_y}.
